Sockpuppet Detection in Wikipedia: A Corpus of Real-World Deceptive Writing for Linking Identities

This paper describes the corpus of sockpuppet cases we gathered from Wikipedia. A sockpuppet is an online user account created with a fake identity for the purpose of covering abusive behavior and/or subverting the editing regulation process. We used a semi-automated method for crawling and curating a dataset of real sockpuppet investigation cases. To the best of our knowledge, this is the first corpus available on real-world deceptive writing. We describe the process for crawling the data and some preliminary results that can be used as baseline for benchmarking research. The dataset will be released under a Creative Commons license from our project website: http://docsig.cis.uab.edu.

==> aa.tex <==

@inproceedings{ArgamonAndJuola:11,
author = {Shlomo Argamon and Patrick Juola},
editor = {},
title = {Overview of the International Authorship Identification Competition at {PAN}-2011},
booktitle = {Proceedings of the PAN 2011 Lab 
Uncovering Plagiarism, Authorship, and Social Software Misuse,
held in conjunction with the CLEF 2011 Conference on Multilingual and Multimodal Information Access Evaluation },
year = {2011},
address = {Amsterdam},
}


@InProceedings{escalante:2011,
  author    = {Escalante, H. J.  and  Solorio, T.  and  Montes-y-G{\'{o}}mez, M.},
  title     = {Local Histograms of Character N-grams for Authorship Attribution},
  booktitle = {Proceedings of the 49th Annual Meeting of the Association for Computational Linguistics: Human Language Technologies},
  month     = {June},
  year      = {2011},
  address   = {Portland, Oregon, USA},
  publisher = {Association for Computational Linguistics},
  pages     = {288--298},

}

@inproceedings{Goldstein-StewartEtAl:08,
  author    = {Jade Goldstein-Stewart and
               Kerri A. Goodwin and
               Roberta Evans Sabin and
               Ransom K. Winder},
  title     = {Creating and Using a Correlated Corpus to Glean Communicative
               Commonalities},
  booktitle = {Proceedings of {LREC-2008}, the Sixth International Language Resources and Evaluation Conference},
  year      = {2008},
}

@inproceedings{Juola:12,
author = {Patrick Juola},
editor = {},
title = {An Overview of the Traditional Authorship Attribution Subtask},
booktitle = {PAN 2012 Lab, Uncovering Plagiarism, Authorship and Social Software Misuse, held in conjunction with CLEF 2012},
year = {2012},
}


@article{LewisEtAl:04,
 author = {Lewis, David D. and Yang, Yiming and Rose, Tony G. and Li, Fan},
 title = {RCV1: A New Benchmark Collection for Text Categorization Research},
 journal = {J. Mach. Learn. Res.},
 volume = {5},
 month = {December},
 year = {2004},
 issn = {1532-4435},
 pages = {361--397},
 numpages = {37},
 acmid = {1005345},
 publisher = {JMLR.org},
} 


@inproceedings{LuyckxAndDaelemans:08,
author = {Kim Luyckx and Walter Daelemans},
editor = {},
title = {Personae: a corpus for author and personality prediction from text.},
booktitle = {Proceedings of LREC-2008, the Sixth International Language Resources and Evaluation Conference},
year = {2008},
}

@inproceedings{NovakEtAl:04,
 author = {Novak, Jasmine and Raghavan, Prabhakar and Tomkins, Andrew},
 title = {Anti-aliasing on the web},
 booktitle = {Proceedings of the 13th international conference on World Wide Web},
 series = {WWW '04},
 year = {2004},
 isbn = {1-58113-844-X},
 location = {New York, NY, USA},
 pages = {30--39},
 numpages = {10},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {alias detection, aliases, bulletin boards, personas, privacy, pseudonyms},
} 


@INPROCEEDINGS{PlakiasAndStamatatos:08,
  AUTHOR =       {S. Plakias and E. Stamatatos},
  TITLE =        {Tensor space models
for authorship attribution},
  BOOKTITLE =    {Proceedings of the 5th
Hellenic Conference on Artificial Intelligence: Theories,
Models and Applications},
  YEAR =         {2008},
  editor =       {},
  volume =       {5138},
  number =       {},
  series =       {LNCS},
  pages =        {239--249},
  address =      {Syros, Greece},
  month =        {},
  organization = {},
  publisher =    {},
  note =         {},
  abstract =     {},
  keywords =     {},
}

@BOOK{witten:2005,
	  AUTHOR =       {I. H. Witten and E. Frank},
	  editor =       {},
	  TITLE =        {Data Mining: Practical Machine Learning Tools and Techniques},
	  PUBLISHER =    {Morgan Kauffmann},
	  YEAR =         {2005},
	  volume =       {},
	  number =       {},
	  series =       {},
	  address =      {},
	  edition =      {2nd},
	  month =        {},
	  note =         {},
	  abstract =     {},
	  isbn =         {},
	  price =        {},
	  keywords =     {},
	  source =       {},
}

@ARTICLE{Stamatatos:08b,
  AUTHOR =       {E. Stamatatos},
  TITLE =        {Author Identification: Using Text Sampling to Handle the Class Imbalance
Problem},
  JOURNAL =      {Information Processing and Managemement},
  YEAR =         {2008},
  volume =       {44},
  number =       {},
  pages =        {790--799},
  month =        {},
  note =         {},
  abstract =     {},
  keywords =     {},
  source =       {},
}


